Local convergence of a sequential quadratic programming method for a class of nonsmooth nonconvex objectives

A sequential quadratic programming (SQP) algorithm is designed for nonsmooth optimization problems with upper-C^2 objective functions. Upper-C^2 functions are locally equivalent to difference-of-convex (DC) functions with smooth convex parts. They arise naturally in many applications such as certain classes of solutions to parametric optimization problems, e.g., recourse of stochastic programming, and projection onto closed sets. The proposed algorithm conducts line search and adopts an exact penalty merit function. The potential inconsistency due to the linearization of constraints are addressed through relaxation, similar to that of Sl_1QP. We show that the algorithm is globally convergent under reasonable assumptions. Moreover, we study the local convergence behavior of the algorithm under additional assumptions of Kurdyka-{\L}ojasiewicz (KL) properties, which have been applied to many nonsmooth optimization problems. Due to the nonconvex nature of the problems, a special potential function is used to analyze local convergence. We show that under acceptable assumptions, upper bounds on local convergence can be proven. Additionally, we show that for a large number of optimization problems with upper-C^2 objectives, their corresponding potential functions are indeed KL functions. Numerical experiment is performed with a power grid optimization problem that is consistent with the assumptions and analysis in this paper.

==> Sections_journal/Algorithm_sto_2.tex <==
This is wrong unfortunately.
\section{\normalsize SQP in deterministic setting}\label{sec:alg}
Motivated by the discussion in Section~\ref{sec:prob}, we make the following assumption. 
\begin{assumption}\label{assp:upperC2}
	The objective $r(\cdot)$ in~\eqref{eqn:opt0} is Lipschitz continuous and upper-$\Ctwo$. 
\end{assumption}
\noindent In particular, inequality~\eqref{eqn:uppc2-def} is satisfied.
Next, we formalize the smoothness of the constraints, a common assumption in literature~\cite{curtis2012}.
\begin{assumption}\label{assp:boundedHc}
	The functions $c(\cdot)$ are continuously differentiable with Lipshitz continuous gradient, or sometimes called L-smooth. This means that there exists a constant $H\geq 0$ such that 
\begin{equation} \label{eqn:l-smooth-constraint}
 \centering
  \begin{aligned}
	  |c_j(x') - c_j(x) - \nabla c_j(x)^T (x'-x) | \leq&  \frac{H}{2} \norm{x-x'}^2, \\
  \end{aligned}
\end{equation}
	for all feasible $x,x'$ and all $j\in\{1, 2, \ldots, m\}$~\cite{nesterovconvex2003}.
\end{assumption}

\subsection{Algorithm description}\label{sec:alg-1}
As in other SQP methods, the objective is approximated with a local quadratic function $\phi_k(\cdot)$ at the $k$th iteration 
and the constraints are linearized. At iteration $k$ and its serious step $x_k$, $\phi_k(\cdot)$ is
\begin{equation} \label{eqn:opt-rc-appx-x}
 \centering
  \begin{aligned}
	  \phi_k(x) = r(x_k) + g_k^T(x-x_k) + \frac{1}{2}(x-x_k)^T B_k (x-x_k),
  \end{aligned}
\end{equation}
where $g_k\in\bar{\partial} r(x_k)$, and $B_k$ is a bounded, symmetric and positive semidefinite matrix.
Equivalently, denoting $d=x-x_k$, $\phi_k(x)$ can be rewritten as $\Phi_k(d)$: 
\begin{equation} \label{eqn:opt-rc-appx}
 \centering
  \begin{aligned}
	  \Phi_k(d) &= r(x_k) + g_k^T d +\frac{1}{2} d^T B_k d.\\ 
  \end{aligned}
\end{equation}
The function 
value and subgradient at $x_k$ are exact, \textit{i.e.}, $\Phi_k(0)=r(x_k),\nabla\Phi_k(0)=g_k$.
The optimization subproblem is
\begin{equation} \label{eqn:opt-ms-simp-bundle}
 \centering
  \begin{aligned}
   &\underset{\substack{d}}{\text{minimize}} 
	  & & \Phi_k(d)\\
   &\text{subject to}
	  & & c(x_k) + \nabla c(x_k)^T d= 0, \ \ \  x_u-x_k\geq d \geq -x_k ,
  \end{aligned}
\end{equation}
where $d_l^k=-x_k,d_u^k=x_u-x_k$.
It is possible that the linearized constraints 
in~\eqref{eqn:opt-ms-simp-bundle} are infeasible. 
Hence, the algorithm solves the following relaxed quadratic programming problem:
\begin{equation} \label{eqn:opt-sqp-penal}
 \centering
  \begin{aligned}
   &\underset{\substack{d,v,w}}{\text{min}} 
	  & & \Phi_k(d) +\theta_k \sum_{j=1}^m (v_j + w_j)  \\
   &\text{s.t.}
	  & & c_j(x_k)+\nabla c_j(x_k)^T d = v_j - w_j, \ j=1,\ldots,m,\\
	  &&& x_u-x_k \geq d\geq -x_k, \ \ v, w \geq 0,
  \end{aligned}
\end{equation}
where $v,w\in \Rbb^m$ are slack variables and $\theta_k>0$ is a penalty parameter. Let $d_k$, $v^k$, and $w^k$ denote the solutions to~\eqref{eqn:opt-sqp-penal}.
The first-order optimality conditions of problem~\eqref{eqn:opt-sqp-penal} for $d_k$ are
\begin{equation} \label{eqn:sqp-penal-KKT-1}
  \centering
   \begin{aligned}
	   g_k + B_k d_k + \sum_{i=1}^m \lambda^{k+1}_j \nabla c_j(x_k)-\zeta_l^{k+1}+\zeta_u^{k+1} =0&,\\
	   c_j(x_k)+\nabla c_j(x_k)^T d_k - v^k_j + w^k_j =0, \ j=1,...m,\\
	   Z_u^{k+1}(d_k+x_k-x_u) = 0, Z_l^{k+1}(d_k+x_k) = 0&,\\
	   \zeta_u^{k+1},\zeta_l^{k+1},d_k+x_k,x_u-x_k-d_k\geq 0&.\\
   \end{aligned}
 \end{equation}
Here, $\lambda^{k+1}\in\Rbb^m$, $\zeta_u^{k+1}\in \Rbb^n$, and $\zeta_l^{k+1}\in \Rbb^n$ are the Lagrange multipliers for the constraints, while $Z_u^{k+1}$ and $Z_l^{k+1}$ are diagonal matrices with values $\zeta_u^{k+1}$ and $\zeta_l^{k+1}$, respectively.
The remaining optimality conditions on slack variables $v^k$ and $w^k$ are 
\begin{equation} \label{eqn:sqp-penal-KKT-2}
  \centering
   \begin{aligned}
	   \theta_k-\lambda^{k+1}_j - p^{k+1}_j =0, \ j=1,...m,\\
           \theta_k+\lambda^{k+1}_j-q^{k+1}_j=0, \ j=1,...m,\\
	   P^{k+1} v^k  = 0, Q^{k+1} w^k = 0&,\\
	   v^k,w^k,p^{k+1},q^{k+1} \geq 0&,\\
   \end{aligned}
 \end{equation}
where $p^{k+1}\in\Rbb^m$ and $q^{k+1}\in\Rbb^m$ are the Lagrange multipliers for bound constraints on $v^k$ and $w^k$, respectively, while $P^{k+1}$ and $Q^{k+1}$ are diagonal matrices with diagonal vector $p^{k+1}$ and $q^{k+1}$, respectively. 


To measure progress in both the objective and constraints, 
a $l_1$ merit function is adopted in the form of
\begin{equation} \label{eqn:opt-sqp-merit}
 \centering
  \begin{aligned}
	  \phi_{1}(x,\theta_k) = r(x) + \theta_k \norm{c(x)}_1, \\
  \end{aligned}
\end{equation}
where $\norm{\cdot}_1$ is the standard 1-norm. 


Let the line search step size be $\alpha_k \in (0,1]$. 
Then, the next step taken is given as 
$x_{k+1} = x_k + \alpha_k d_k$.
Given the equality constraint, we adopt the following line search criterion: 
\begin{equation}\label{eqn:line-search-cond}
   \begin{aligned}
   \centering
       \phi_1(x_k,\theta_k) - \phi_1(x_{k+1},\theta_k) 
	   \geq \eta \alpha_k \frac{1}{2} d_k^T B_k d_k, 
   \end{aligned}
\end{equation}
where $\eta\in (0,1)$ is the line search coefficient.

To proceed, we define the sign function $\sigma_j^k:\Rbb^n\to\Rbb$, $j=1,\dots,m$ of $d$ 
based on whether the slack variable bound constraints are active:
\begin{equation} \label{eqn:opt-sqp-sign}
 \centering
  \begin{aligned}
	  \sigma_j^k(d)  =  
	  \begin{cases}
		  -1,  
		       & c_j(x_k)+\nabla c_j(x_k)^T d < 0, \\  
		  \phantom{-}0,
		  & c_j(x_k) + \nabla c_j(x_k)^T d = 0,\\
		  \phantom{-}1,
		  & c_j(x_k) + \nabla c_j(x_k)^T d > 0.
    \end{cases}
  \end{aligned}
\end{equation}
In addition, for $d_k$, we define
%we divide the constraints into two sets based on the value of $ c_j(x_k)+ \nabla c_j(x_k)^T d_{k}$. 
%For simplicity, the two sets are referred to as the set of active and inactive equality constraints as we do without slack variables. 
the active equality constraint set as
\begin{equation} \label{eqn:opt-sqp-fea-A}
   \centering
    \begin{aligned}
     A_k = \{ 1\leq j\leq m|c_j(x_k)+\nabla c_j(x_k)^T d_{k} = 0\},
     \end{aligned}
\end{equation}
and the inactive equality constraint set as
\begin{equation} \label{eqn:opt-sqp-fea-I}
  \centering
    \begin{aligned}
      V_k = \{ 1\leq j\leq m|c_j(x_k)+\nabla c_j(x_k)^T d_{k} \neq 0\}.
    \end{aligned}
\end{equation}
%		  %
Our nonsmooth line search SQP algorithm is presented in Algorithm~\ref{alg:sqp}, where $\norm{\cdot}_{\infty}$ is the infinity norm. 
\begin{algorithm}
% \DontPrintSemicolon
% \SetAlgoNoLine 
   \caption{Nonsmooth SQP with line search}\label{alg:sqp}
	\begin{algorithmic}[1]
	    \STATE{Initialize $x_0$, $B_0$, $\theta_0$, stopping error tolerance $\epsilon$, $\epsilon_c$, and $k=0$.
		Choose scalars $0<\eta < 1$, $\tau_{\alpha}\in (0,1)$ and $\gamma>0$. }
	\FOR{$k=0,1,2,...$}
	  \STATE{Evaluate the function value $f(x_k)$ and subgradient $g_k\in \bar{\partial}f(x_k)$.}
	  \STATE{Form the quadratic function $\Phi_k$ in~\eqref{eqn:opt-rc-appx} and solve 
		subproblem~\eqref{eqn:opt-sqp-penal} to obtain $d_{k}$ and Lagrange multiplier $\lambda^{k+1}$.} 
	  \IF{$\norm{d_k}\leq \epsilon$ \text{and} $\norm{c(x_k)}_{\infty}\leq \epsilon_c$}
	    \STATE{Stop the iteration and exit the algorithm.}
	  \ENDIF
	   \STATE{Set $\theta_{k+1} = \max{\{\theta_{k-1}, \norm{\lambda^{k+1}}_{\infty}+\gamma\}}$. }
	   \STATE{Find the line search step size $\alpha_k>0$ using backtracking, starting at $\alpha_k=1$ and reducing $\alpha_k$ by 
		$\alpha_k = \tau_{\alpha} \alpha_k$ until the conditions in~\eqref{eqn:line-search-cond} are satisfied.}
           \STATE{Take the step $x_{k+1} = x_k+\alpha_k d_k$.}
	    \STATE{Call the chosen $B_k$ update rules to obtain $B_{k+1}$.}
       \ENDFOR
    \end{algorithmic}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Convergence
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Convergence analysis}\label{sec:alg-convg}
If the algorithm terminates in a finite number of steps, the stopping test at step 4 is satisfied with the error tolerance $\epsilon,\epsilon_c$ and the solution is considered found. 
Let $\epsilon=\epsilon_c=0$, then $\norm{d_k}= 0$ and $\norm{c(x_k)}_{\infty}=0$.
Since $d_k$ solves~\eqref{eqn:opt-sqp-penal}, optimality conditions in~\eqref{eqn:sqp-penal-KKT-1}
are satisfied, of which the first equation reduces to 
\begin{equation}\label{alg:finite-steps}
 \begin{aligned}
	 g_k + \nabla c(x_k) \lambda^{k+1}-\zeta_l^{k+1}+\zeta_u^{k+1}=0.
 \end{aligned}
\end{equation}
Given $g_k\in\bar{\partial} r(x_k)$, we have $0\in \bar{\partial} r(x_k)+\nabla c(x_k) \lambda^{k+1}-\zeta_l^{k+1}+\zeta_u^{k+1}$. 
In addition,  from $c(x_k) = 0$, $x_k$ is feasible as the bound constraints are enforced in the subproblem~\eqref{eqn:opt-sqp-penal}.
From the remaining equations in~\eqref{eqn:sqp-penal-KKT-1} 
and~\eqref{eqn:sqp-penal-KKT-2}, $x_k$ satisfies~\eqref{eqn:opt0-KKT} and is by definition a KKT point for~\eqref{eqn:opt0} as the algorithm exits.
In what follows, the analysis is focused on the case with an infinite number of steps, \textit{i.e.}, $\norm{d_k}>0$ or $\norm{c(x_k)}_{\infty}>0$. 
Further, Assumptions~\ref{assp:upperC2} and~\ref{assp:boundedHc} are assumed valid throughout the anlysis.

We start with the following lemma that establishes the relationship between $\lambda^{k+1}$ and $\theta_k$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lem:lambda-sqp-prop}
	For all $j\in V_k$, $\lambda_j^{k+1} = \sigma_j^k(d_k)\theta_k$. Also, for all $j\in A_k$, 
        $\lambda_j^{k+1}\in [-\theta_k,\theta_k]$.
\end{lemma}
\begin{proof}
	Note first that for any $ j\in[1,m]$, the slack variable solutions satisfy $v^k_j w^k_j = 0$. 
	We consider the three cases given by the value of $\sigma_j^k(d_k),j=1,\dots,m$.
	If $\sigma_j^k(d_k)=1$, by the second equation in~\eqref{eqn:sqp-penal-KKT-1}, $v_j^k>0$ and $w_j^k=0$.
	From the third line in~\eqref{eqn:sqp-penal-KKT-2}, 
        $p^{k+1}_j=0$. Then, by the first equation in~\eqref{eqn:sqp-penal-KKT-2}, $\lambda_j^{k+1}=\theta_k$.
	Similarly, if $\sigma_j^k(d_k)=-1$, 
        one obtains $q^{k+1}_j=0$ and $\lambda_j^{k+1}=-\theta_k$. The first part of the Lemma is proven.

	In the last case, $j\in A_k$, \textit{i.e.}, $\sigma_j^k(d_k)=0$. By the second equation in~\eqref{eqn:sqp-penal-KKT-1}, we have $v_j^k=0$ and $w_j^k=0$.  
We sum and subtract the first two equations in~\eqref{eqn:sqp-penal-KKT-2} to obtain 
%      \begin{equation} \label{eqn:lambda-pq}
%       \centering
%        \begin{aligned}
		$\lambda_j^{k+1} = \frac{1}{2}(q_j^{k+1}-p_j^{k+1})$ and %\\
		$p_j^{k+1}+q_j^{k+1}=2\theta_k$. %\\
        %\end{aligned}
       %\end{equation}
	The bound constraints on $p^{k+1}$ and $q^{k+1}$ and the latter equation implies $0\leq p_j^{k+1}$ and $q_j^{k+1}\leq 2\theta_k$; finally,
	the former equation implies $\lambda_j^{k+1}\in [-\theta_k,\theta_k]$.
\end{proof}

\begin{remark}\label{rmrk:realalpha}
	We do not specify how $B_k$ is specifies in this paper. Given the nonsmooth nature of $f(\cdot)$, 
        an approximation to Hessian is not possible. 
	We do encourage a diagonal matrix so that the sparsity structure of the linear system is perserved~\cite{wang2022}.
\end{remark}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lem:line-search-cons}
	Given the Lagrange multipliers $\lambda^{k+1}$, the constraints part of the merit function satisfies the following inequality 
       \begin{equation} \label{eqn:line-search-cons-ineq}
         \centering
         \begin{aligned}
	    \theta_k\norm{c(x_k)}_1 - \theta_k\norm{c(x_{k+1})}_1 + \alpha_k \sum_{j=1}^m \lambda^{k+1}_j\nabla c_j(x_k)^T d_k
                     \geq -  \frac{1}{2}\theta_k \alpha_k^2 c_h \norm{d_k}^2,
      \end{aligned}
     \end{equation}
	where $c_h>0$ is a constant coefficient.
\end{lemma}
\begin{proof}
	By Assumption~\ref{assp:boundedHc}, for $x_{k+1}=x_k+\alpha_k d_k$ and $1\leq j \leq m$,
       \begin{equation} \label{eqn:sqp-c-ls-pf-1}
         \centering
         \begin{aligned}
		 |c_j(x_{k+1})  - c_j(x_k)- \alpha_k \nabla c_j(x_k)^T d_{k}| \leq \frac{1}{2}\alpha_k^2 H \norm{d_k}^2.\\
      \end{aligned}
     \end{equation}
	By triangle inequality, we have
   \begin{equation} \label{eqn:sqp-c-ls-pf-2}
   \centering
    \begin{aligned}
	    |c_j(x_{k+1})|  
	    &\leq | c_j(x_k) + \alpha_k \nabla c_j(x_k)^T d_{k}| + \frac{1}{2}\alpha_k^2 H \norm{d_k}^2\\
	     &= \left|(1-\alpha_k) c_j(x_k) + \alpha_k \left[c_j(x_k)+ \nabla c_j(x_k)^T d_{k}\right]\right|+\frac{1}{2}\alpha_k^2 H \norm{d_k}^2\\ 
	      & \leq (1-\alpha_k)| c_j(x_k)| + \alpha_k |c_j(x_k)+ \nabla c_j(x_k)^T d_{k}|+ \frac{1}{2}\alpha_k^2 H \norm{d_k}^2 . 
    \end{aligned}
   \end{equation}
	Applying the definition~\eqref{eqn:opt-sqp-sign} of $\sigma_j^k$ to~\eqref{eqn:sqp-c-ls-pf-2}, we can write 
\begin{equation} \label{eqn:sqp-c-ls-pf-2.3}
   \centering
    \begin{aligned}
	    |c_j(x_{k+1})|  
		  & \leq (1-\alpha_k)|c_j(x_k)| + \alpha_k \sigma_j^k(d_k)\left[c_j(x_k)+ \nabla c_j(x_k)^T d_{k}\right] + \frac{1}{2}\alpha_k^2 H\norm{d_k}^2.
    \end{aligned}
   \end{equation}
	Let us denote the cardinality of $A_k$ and $V_k$ by $|A_k|$ and $|V_k|$, respectively. By summing up~\eqref{eqn:sqp-c-ls-pf-2.3} over $j\in V_k$ and noting that $|c_j(x_k)|\geq \sigma_j^k(d_k) c_j(x_k)$, we have
   \begin{equation} \label{eqn:sqp-c-ls-pf-2.5}
     \centering
      \begin{aligned}
	      \sum_{j\in V_k}|c_j(x_{k+1})|  \leq& 
	       \sum_{j \in V_k}  |c_j(x_k)|+\alpha_k\sum_{j \in V_k} \sigma_j^k(d_k)\nabla c_j(x_k)^Td_k 
	      + \frac{1}{2}|V_k|\alpha_k^2 H \norm{d_k}^2.\\
      \end{aligned}
    \end{equation}
	Similarly, we sum up~\eqref{eqn:sqp-c-ls-pf-2.3} over $j\in A_k$ and use the definition in~\eqref{eqn:opt-sqp-fea-A} to write 
   \begin{equation} \label{eqn:sqp-c-ls-pf-2.6}
     \centering
      \begin{aligned}
\sum_{j\in A_k}|c_j(x_{k+1})|  \leq& 
	      (1-\alpha_k)\sum_{j \in A_k}  |c_j(x_k)| + \frac{1}{2}|A_k| \alpha_k^2 H \norm{d_k}^2. \\
      \end{aligned}
    \end{equation}
    Summing the two equations in~\eqref{eqn:sqp-c-ls-pf-2.5} and~\eqref{eqn:sqp-c-ls-pf-2.6}
    and using $|A_k|+|V_k|=m$ gives us 
\begin{equation} \label{eqn:sqp-c-ls-pf-3}
     \centering
      \begin{aligned}
	      \norm{c(x_k)}_1-\norm{c(x_{k+1})}_1 \geq  
	    \alpha_k  \sum_{j \in A_k}  |c_j(x_k)|   -\alpha_k \sum_{j \in V_k} \sigma_j^k(d_k)\nabla c_j(x_k)^T d_k 
	      - \frac{1}{2}m\alpha_k^2 H \norm{d_k}^2. \\
      \end{aligned}
    \end{equation}
    From Lemma~\ref{lem:lambda-sqp-prop} and the definition~\eqref{eqn:opt-sqp-fea-A} of $A_k$, we can write
\begin{equation} \label{eqn:sqp-c-ls-pf-3.1}
     \centering
      \begin{aligned}
	      \sum_{j=1}^m \lambda_j^{k+1}\nabla c_j(x_k)^T d_k =& \sum_{j\in V_k} \lambda_j^{k+1} \nabla c_j(x_k)^T d_k +\sum_{j\in A_k} \lambda_j^{k+1} \nabla c_j(x_k)^T d_k\\
	      =& \sum_{j\in V_k} \sigma_j^k(d_k)\theta_k \nabla c_j(x_k)^T d_k -\sum_{j\in A_k} \lambda^{k+1}_j  c_j(x_k).\\
	      \geq& \sum_{j\in V_k} \sigma_j^k(d_k)\theta_k \nabla c_j(x_k)^T d_k - \theta_k\sum_{j\in A_k}  |c_j(x_k)|.\\
      \end{aligned}
    \end{equation}
    The inequality in~\eqref{eqn:sqp-c-ls-pf-3.1} comes from the second part of Lemma~\ref{lem:lambda-sqp-prop}, 
    namely $\lambda^{k+1}_j\in [-\theta_k,\theta_k]$.
	Through basic algebraic calculations and applying~\eqref{eqn:sqp-c-ls-pf-3.1} to~\eqref{eqn:sqp-c-ls-pf-3}, 
   \begin{equation} \label{eqn:sqp-c-ls-pf-3.5}
   \centering
    \begin{aligned}
	    &  \theta_k\norm{c(x_k)}_1 - \theta_k\norm{c(x_{k+1})}_1 + \alpha_k \sum_{j=1}^m \lambda^{k+1}_j\nabla c_j(x_k)^T d_k
	     \geq \\
	    &\qquad \theta_k \alpha_k \sum_{j \in A_k}  |c_j(x_k)|  
	      -\theta_k \alpha_k  \sum_{j \in V_k} \sigma_j^k(d_k)\nabla c_j(x_k)^T d_k
	      - \frac{1}{2} \theta_k m\alpha_k^2 H \norm{d_k}^2 \\ 
	    & \qquad+ \alpha_k\theta_k\sum_{j\in V_k} \sigma_j^k(d_k) \nabla c_j(x_k)^T d_k
	     - \alpha_k \theta_k\sum_{j\in A_k} | c_j(x_k) | \geq 
	    -  \frac{1}{2}\theta_k m \alpha_k^2 H \norm{d_k}^2.
    \end{aligned}
   \end{equation}
    Let $c_h = mH$ to complete the proof.
\end{proof}

\begin{lemma}\label{lem:line-search-merit}
	If the Lagrange multipliers $\lambda^{k+1}$ are bounded, then step 8 of Algorithm~\ref{alg:sqp} finds $\alpha_k\in (0,1]$ satisfying the line search condition~\eqref{eqn:line-search-cond} in a finite number of steps.
\end{lemma}

\begin{proof}
      By Assumption~\ref{assp:upperC2}, we have  
	\begin{equation} \label{eqn:sqp-merit-penal-pf-1}
 \centering
  \begin{aligned}
	  r(x_k) - r(x_{k+1}) >& -\alpha_k g_{k}^Td_k -\frac{\rho}{2}  \alpha_k^2 \norm{d_k}^2. \\
  \end{aligned}
\end{equation}
	Let us rearrange the first equation in the KKT conditions~\eqref{eqn:sqp-penal-KKT-1} to obtain 
\begin{equation} \label{eqn:sqp-penal-merit-pf-1}
  \centering
   \begin{aligned}
	    g_k + B_k d_k  = -\sum_{j=1}^m\lambda_j^{k+1} \nabla c_j(x_k) 
	     + \zeta_l^{k+1}-\zeta_u^{k+1}.\\
   \end{aligned}
 \end{equation}
	Taking the dot product with $-d_k$ on both sides of~\eqref{eqn:sqp-penal-merit-pf-1} leads to
\begin{equation} \label{eqn:sqp-penal-merit-pf-2}
  \centering
   \begin{aligned}
	   - g_k^Td_k - d_k^T B_k d_k =& \sum_{j=1}^m\lambda^{k+1}_j \nabla c_j(x_k)^T d_k 
	    -d_k^T \zeta_l^{k+1} + d_k^T \zeta_u^{k+1}.\\
   \end{aligned}
 \end{equation}
	Recall that $d_l^k=-x_k$ and $d_u^k=x_u-x_k$.
	Using the third and fourth equations in~\eqref{eqn:sqp-penal-KKT-1}, we have
\begin{equation} \label{eqn:sqp-penal-merit-pf-2.3}
  \centering
   \begin{aligned}
	   -d_k^T \zeta_l^{k+1} + d_k^T \zeta_u^{k+1} =& -(d_k+x_k-x_k)^T\zeta_l^{k+1}+(d_k+x_k-x_u-x_k+x_u)^T\zeta_u^{k+1}\\
					       =& x_k^T \zeta_l^{k+1} +(x_u-x_k)^T \zeta_u^{k+1}
					       \geq 0.
   \end{aligned}
 \end{equation}
	The inequality above uses the bound constraints, namely, $0\leq x_k\leq x_u$, $\zeta_u^{k+1}\geq 0$, and $\zeta_l^{k+1}\geq 0$.
	Applying~\eqref{eqn:sqp-penal-merit-pf-2.3}  to~\eqref{eqn:sqp-penal-merit-pf-2}, we have
\begin{equation} \label{eqn:sqp-penal-merit-pf-2.5}
  \centering
   \begin{aligned}
	   -g_k^Td_k  
	   \geq & d_k^T B_k d_k +\sum_{j=1}^m \lambda_j^{k+1} \nabla c_j(x_k)^T d_k.\\
   \end{aligned}
 \end{equation}
	Since $\alpha_k\in (0,1]$, one can multiply~\eqref{eqn:sqp-penal-merit-pf-2.5} by $\alpha_k$ and
	apply it to~\eqref{eqn:sqp-penal-merit-pf-1} to obtain
\begin{equation} \label{eqn:sqp-penal-merit-pf-3}
  \centering
   \begin{aligned}
	   f(x_k) - f(x_{k+1}) \geq \alpha_k d_k^T B_k d_k -\frac{\rho}{2}\alpha_k^2\norm{d_k}^2 + \alpha_k \sum_{j=1}^m \lambda_j^{k+1} \nabla c_j(x_k)^T d_k
   \end{aligned}
 \end{equation}
	From Lemma~\ref{lem:line-search-cons}, Assumption~\ref{}, and~\eqref{eqn:sqp-penal-merit-pf-3}, the merit function satisfies
\begin{equation*}% \label{eqn:simp-bundle-penal-merit-pf-4} 
 \centering
  \begin{aligned}
	  \phi_{1}&(x_k,\theta_k) - \phi_{1}(x_{k+1},\theta_k)  = f(x_k) -f(x_{k+1})+ \theta_k\norm{c(x_k)}_1
		    -\theta_k\norm{c(x_{k+1})}_1\\
			 \geq & \alpha_k d_k^TB_kd_k - \frac{\rho}{2} \alpha_k\norm{d_k}^2+ \alpha_k \sum_{j=1}^m \lambda_j^{k+1} \nabla c_j(x_k)^T d_k + \theta_k\norm{c(x_k)}_1
		    -\theta_k\norm{c(x_{k+1})}_1\\
			\geq& \frac{1}{2}\alpha_k d_k^TB_kd_k + \frac{\alpha_k}{2} (b- \rho \alpha_k - \theta_k \alpha_k c_h)  \norm{d_k}^2. \\
  \end{aligned}
\end{equation*}
 Since $\lambda^k$ is bounded, 
 there exists $k$ such that $\theta_t=\theta_k>0$ for all $t\geq k$.
 Then step 8 line search completes successfully once $b>(\rho+\theta_k c_h)\alpha_k$ is achieved by reducing $\alpha_k$. 

\end{proof}

In order to attain bounded Lagrange multipliers, a constraint qualification is necessary 
for $c(\cdot)=0$ in~\eqref{eqn:opt0}.
Given the existence of both equality and inequality constraints, we resort to the Mangasarian-Fromovitz constraint qualificatin (MFCQ)~\cite{Nocedal_book}.
Denote by $e_i \in \Rbb^n$ the unit vector where $(e_i)_i = 1$ and $(e_i)_l = 0,l\neq i$, the MFCQ is defined below.
\begin{definition}\label{assp:MFCQ}
	The constraints in~\eqref{eqn:opt0} satisfy MFCQ at $x$ if the gradients $\nabla c_j(x)$, $j=1,\dots,m$ are linearly independent and there exists a vector $w\in \Rbb^n$ such that 
  \begin{equation}\label{def:mfcq}
   \centering
    \begin{aligned}
	e_i^T w >0, i \in I_l, \ e_i^T w <0, i \in I_u, \ \nabla c_j(x)^T w = 0, j=1,\dots,m,
    \end{aligned}
  \end{equation}
	where $I_l$ and $I_u$ are index sets such that $x_i=0$ for all $i\in I_l$ and $x_i=x_u$ for all $i\in I_u$.
\end{definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lem:bounded-lp}
	If MFCQ of the constraints in~\eqref{eqn:opt0} are satisfied at every accumulation points $\bar{x}$ of serious steps $\{x_k\}$ generated by the algorithm, then 
	the sequence of Lagrange multipliers for problem~\eqref{eqn:opt-ms-simp-bundle} $\{\zeta_u^{k+1}\},\{\zeta_l^{k+1}\}$ and $\{\lambda^{k+1}\}$ are bounded. 
	In addition, this means there exists $k$ such that $\theta_t = \theta_k$ for all $t\geq k$.
\end{lemma}
\begin{proof}
     We rewrite the first equation in optimality condition in~\eqref{eqn:sqp-penal-KKT-1} as
    \begin{equation} \label{eqn:sqp-penal-KKT-full}
     \centering
     \begin{aligned}
	     g_k + B_k d_k + \sum_{j=1}^m \lambda^{k+1}_j \nabla c_j(x_k) -\sum_{i=1}^n (\zeta_l^{k+1})_i e_i 
	     +\sum_{i=1}^n (\zeta_u^{k+1})_i e_i &=0,\\
     \end{aligned}
    \end{equation}
    The Lagrange multipliers for the bound constraints can be combined into one vector $\zeta^{k+1}=\zeta_l^{k+1}- \zeta_u^{k+1}$,
    since $(\zeta_l^{k+1})_i(\zeta_u^{k+1})_i = 0$.
	A component of $\zeta_l^{k+1}$ or $\zeta_u^{k+1}$ is unbounded if and only if the corresponding component in $\zeta^{k+1}$ is unbounded.
	Let $I_l^k$ and $I_u^k$ be the index sets of the active bound constraints for the lower and upper bounds at iteration $k$. We have 
    \begin{equation} \label{eqn:sqp-bnd-multi}
     \centering
     \begin{aligned}
	     I_l^k \cap I_u^k = \emptyset, \ \zeta^{k+1}_j>0 \ \text{for} \ j\in I_l, \ \zeta^{k+1}_j <0 \ \text{for} \ j \in I_u.
     \end{aligned}
    \end{equation}
	Consequently,~\eqref{eqn:sqp-penal-KKT-full} can be written as
    \begin{equation} \label{eqn:sqp-penal-KKT-full-2}
     \centering
     \begin{aligned}
	     g_k + B_k d_k = -\sum_{j=1}^m \lambda^{k+1}_j \nabla c_j(x_k) +\sum_{i \in I^k} (\zeta^{k+1})_i e_i,\\
     \end{aligned}
    \end{equation}
	where $I^k=I_l^k\cup I_u^k$.
	Since $\{x_k\},\{g_k\}$ are bounded and $B_k$ is finite by Assumption~\ref{}, 
	the left-hand side of the equation stays bounded as $k\to\infty$. 

	Suppose contrary to the Lemma, at least one of the Lagrange multipliers is unbounded. 
	Let $t_k = \max\{\norm{\lambda^{k+1}}_{\infty},\norm{\zeta^k}_{\infty}\}$. Then, $t_k\to\infty$ as $k\to \infty$.
	We can thus construct an unbounded subsequence $\{t_{k_u}\}$ that is monotonic. The corresponding subsequences $\{x_{k_u}\}$, $\{g_{k_u}\}$ remain bounded. Passing on to a subsequence if necessary, we can assume $x_{k_u}\to\bar{x}$ as $k\to\infty$, where $\bar{x}$ is an accumulation point. 

	Next, we divide both sides of~\eqref{eqn:sqp-penal-KKT-full-2} by $t_{k_u}$ and obtain
     \begin{equation} \label{eqn:sqp-penal-KKT-full-3}
       \centering
       \begin{aligned}
	       \frac{1}{t_{k_u}} ( g_{k_u} + B_{k_u} d_{k_u} ) = 
	       -\sum_{j=1}^m  a^{k_u+1}_j\nabla c_j(x_{k_u}) 
	       +\sum_{i \in I^k} b^{k_u+1}_i  e_i, 
       \end{aligned}
      \end{equation}
	where $a^{k_u+1}\in\Rbb^m $, $b^{k_u+1}\in\Rbb^n$ are defined as
     \begin{equation} \label{eqn:sqp-penal-multi-2}
       \centering
       \begin{aligned}
	       a^{k_u+1}_j = \frac{\lambda^{k_u+1}_j}{ t_{k_u}}, \ b^{k_u+1}_j =  \frac{(\zeta^{k_u+1})_j}{ t_{k_u}}.
       \end{aligned}
      \end{equation}
	The left-hand side of~\eqref{eqn:sqp-penal-KKT-full-3} converges to $0$ as $k\to\infty$.
	However, depending on the asymptotic behavior of $\lambda^{k_u+1}$ and $\zeta^{k_u+1}$, 
	there are two cases regarding the values of $a^{k_u+1}$ and $b^{k_u+1}$. 
	The first case is where $\norm{\lambda^{k_u}}_{\infty}\to\infty$ and $\norm{\zeta^{k_u}}_{\infty}\leq \norm{\lambda^{k_u}}_{\infty}$. Notice that $\zeta^{k_u}$ can be unbounded.
	Then, there exists $t\in[1,m]$ such that 
	$|a_t^{k_u+1}| = 1$ while $|b^{k_u+1}_j| \to 0$ for all $j=1,\dots,n$. By the linear independence of 
	$\nabla c_j(\bar{x})$ from MFCQ, the right-hand side of~\eqref{eqn:sqp-penal-KKT-full-3} does not converge to zero.
        This is a contradiction.

	The second case is when  $\norm{\zeta^{k_u}}_{\infty}\to\infty$ while $ \norm{\lambda^{k_u}}_{\infty} \leq \norm{\zeta^{k_u}}_{\infty}$. 
        Notice that it is possible $\norm{\lambda^{k_u}}_{\infty}\to\infty$.
	Then, there exists $t\in[1,n]$, such that $|b^{k_u+1}_t|=1$.
	From MFCQ at $\bar{x}$, there exists $w \in \Rbb^n$ such that~\eqref{def:mfcq} is satisfied at $\bar{x}$. Taking the dot product with $w$ on both sides of~\eqref{eqn:sqp-penal-KKT-full-3}, we have  
     \begin{equation} \label{eqn:sqp-penal-KKT-full-5}
       \centering
       \begin{aligned}
	       \frac{1}{t_{k_u}} ( g_{k_u} + \alpha_{k_u} d_{k_u} )^T w = 
	       -\sum_{j=1}^m  a^{k_u+1}_j\nabla c_j(x_{k_u})^T w 
	       +\sum_{i \in I^k} b^{k_u+1}_i  e_i^T w . 
       \end{aligned}
      \end{equation}
      From~\eqref{def:mfcq},~\eqref{eqn:sqp-bnd-multi} and~\eqref{eqn:sqp-penal-multi-2}, at $\bar{x}$, $\bar{b}_i e_i^T w > 0$ for all $i\in \bar{I}$.
      Therefore, the left-hand side of~\eqref{eqn:sqp-penal-KKT-full-5} $\to 0$ while  
     \begin{equation} \label{eqn:sqp-penal-KKT-full-6}
       \centering
       \begin{aligned}
	       -\sum_{j=1}^m  a^{k_u+1}_j\nabla c_j(x_{k_u})^T w 
	       +\sum_{i \in I^k} b^{k_u+1}_i  e_i^T w \to \sum_{i\in\bar{I}} \bar{b}_i e_i^T w > 0. 
       \end{aligned}
      \end{equation}
This is again a contradiction. 

	Therefore, $\{t_k\}$ is bounded and there exist $\lambda^U\geq 0$, $\zeta_l^U\geq 0$, $\zeta_u^U\geq 0$  such that 
	$\norm{\lambda^{k}}_{\infty} \leq \lambda^U$, $\zeta^{k}_u \leq \zeta_u^U$ and $\zeta^{k}_l \leq \zeta_l^U$ for all $k$.
	Since $\theta_k$ is determined by $\lambda^k$, there exists $k$ such that $\theta_t=\theta_k$ for all $t\geq k$. 
\end{proof}

\begin{lemma}\label{lem:merit-decrease}
       If the constraints in~\eqref{eqn:opt0} satisfy the MFCQ 
	conditions in Lemma~\ref{lem:bounded-lp},
	then the merit function sequence $\{\phi_1(x_k,\theta_k)\}$ satisfies  
\begin{equation*} \label{eqn:merit-decrease-1} 
 \centering
  \begin{aligned}
	  \phi_{1}&(x_k,\theta_k) - \phi_{1}(x_{k+1},\theta_k)  
			\geq& \frac{1}{2} c_{\phi} \norm{d_k}^2, \\
  \end{aligned}
\end{equation*}
	for some $c_{\phi}>0$.
\end{lemma}
\begin{proof}
	From Lemma~\ref{lem:line-search-merit}, applying Assumption~\ref{} to~\eqref{eqn:line-search-cond}, we have 
\begin{equation} \label{eqn:merit-decrease-2} 
 \centering
  \begin{aligned}
	  \phi_{1}&(x_k,\theta_k) - \phi_{1}(x_{k+1},\theta_k)  
			\geq& \eta \alpha_k \frac{1}{2} b \norm{d_k}^2. \\
  \end{aligned}
\end{equation}
	From the proof of~\ref{lem:line-search-merit}, once $\alpha_k< b/(\rho+\theta_k c_h)$, the line search exits.
	Using ceiling function $\lceil\cdot \rceil$, which returns the least integer greater than the input, we have  
   \begin{equation} \label{eqn:merit-decrease-3}
   \centering
    \begin{aligned}
	    \alpha_k \geq \tau_{\alpha} ^{\lceil \log_{\tau_{\alpha}} \frac{b }{\rho +\theta_k  c_h} \rceil}.
    \end{aligned}
   \end{equation}
	where $\tau_{\alpha}$ is a parameter from the algorithm. From Lemma~\ref{lem:bounded-lp}, $\{\theta_k\}$ is bounded above.
	Therefore, there exists $\underline{\alpha}>0$ such that $\alpha_k\geq \underline{\alpha}$ for all $k=0,1,2,\dots$.
	Let $c_{\phi} = \eta \underline{\alpha} b$ and the proof is complete.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}\label{thm:simp-KKT}
	If the constraints in~\eqref{eqn:opt0} satisfy the MFCQ 
	conditions in Lemma~\ref{lem:bounded-lp}, then every accumulation point $\bar{x}$ of $\{x_k\}$ generated by Algorithm~\ref{alg:sqp} 
	is a KKT point of the problem~\eqref{eqn:opt0}. 
	That is, there exists a subsequence $\{x_{k_s}\}$ of $\{x_k\}$, where $ x_{k_s} \to \bar{x}$, and $\bar{\lambda}\in\Rbb^m$, $\bar{\zeta}_u\in\Rbb^n$, $\bar{\zeta}_l\in\Rbb^n$, so that the KKT conditions~\eqref{eqn:opt0-KKT} are satisfied at $\bar{x}$.
\end{theorem}
\begin{proof}
	By Lemma~\ref{lem:bounded-lp}, there exists $k_0>0$ such that for $t\geq k_0$, the Lagrange multipliers are bounded above and $\theta_t=\theta_{k_1}=\bar{\theta}$. 
	Let $k\geq k_0$.
	Since $\{x_k\}$ and $\{g_{k}\}$ are bounded, there exists at least one accumulation point for $\{x_k\}$.
	Let $\bar{x}$ be an accumulation point of $\{x_k\}$ and $\{x_{k_s}\}$ be a subsequence of $\{x_k\}$ such that $x_{k_s}\to \bar{x}$.
	From Lemma~\ref{lem:merit-decrease}, we have that
	for $k$ large enough, $\{\phi_{1}(x_k,\theta_k)\}$ is a decreasing and bounded sequence 
	with a fixed parameter $\bar{\theta}$. 
	Thus, $\phi_{1}(x_k,\theta_k)$ converges. 
	
	From Lemma~\ref{lem:merit-decrease},
	we know that $\phi_{1}(x_k,\theta_k)-\phi_{1}(x_{k+1},\theta_k)$ is 
	bounded below in the order of $\norm{d_k}^2$. Therefore,  $\lim_{k\to\infty} \norm{d_k}\to 0$. In particular, $\lim_{s\to \infty}\norm{d_{k_s}}\to 0$.
	From  step 7 in Algorithm~\ref{alg:sqp} we have $\bar{\theta} \geq \lambda_j^{k_s+1} + \gamma$ for $j\in[1,m]$ and $k_s$ large enough. 
	Using the first two equalities in~\eqref{eqn:sqp-penal-KKT-2}, we have $p_j^{k_s+1}\geq \gamma>0$. Passing on to a subsequence if necessary, we assume $p^{k_s} \to \bar{p}>0$, and thus by the third equation in~\eqref{eqn:sqp-penal-KKT-2} $v^{k_s}\to \bar{v} = 0$. Similarly, we have $w^{k_s}\to 0$. From third equation in~\eqref{eqn:sqp-penal-KKT-1}, we have $c(\bar{x}) = 0$.
        Given that the bound constraints are satisfied by all $x_k$, we have $0\leq \bar{x}\leq x_u$. 
          
	Passing on further to a subsequence if necessary, we let $g_{k_s}\to \bar{g}$, 
	$\lambda^{k_{s}+1} \to \bar{\lambda}$, $\zeta_u^{k_{s}+1} \to \bar{\zeta}_u$, $\zeta_l^{k_{s}+1} \to \bar{\zeta}_l$. 
        From the first equation in the optimality conditions~\eqref{eqn:sqp-penal-KKT-1}, we have 
        \begin{equation} \label{eqn:simp-bundle-KKT-limit-1}
          \centering
          \begin{aligned}
		  0 = \bar{g} - \nabla c(\bar{x}) \bar{\lambda}  -\bar{\zeta}_l +\bar{\zeta}_u. 
          \end{aligned}
        \end{equation}
	By the outer semicontinuity of Clarke subdifferential, with $g_{k_s}\in \bar{\partial} r(x_{k_s})$, we have $\bar{g} \in \bar{\partial} r(\bar{x})$.
        As a result, 
	  $0 \in \bar{\partial} r(\bar{x}) -\nabla c(\bar{x}) \bar{\lambda} -\bar{\zeta}_l +\bar{\zeta}_u$.
	The complementarity conditions of bound constraints from~\eqref{eqn:sqp-penal-KKT-1} lead 
	to $\bar{Z}_u(\bar{x}-x_u)$, $\bar{Z}_l\bar{x}=0$. Together with the 
	equality constraints $c(\bar{x}) = 0$, the necessary 
	optimality conditions~\eqref{eqn:opt0-KKT} at $\bar{x}$ are satisfied.
\end{proof}




